Technical Report: A Hierarchical Deliberative-Reactive System Architecture for Task and Motion Planning in Partially Known Environments

We describe a task and motion planning architecture for highly dynamic systems that combines a domain-independent sampling-based deliberative planning algorithm with a global reactive planner. We leverage the recent development of a reactive, vector field planner that provides guarantees of reachability to large regions of the environment even in the face of unknown or unforeseen obstacles. The reachability guarantees can be formalized using contracts that allow a deliberative planner to reason purely in terms of those contracts and synthesize a plan by choosing a sequence of reactive behaviors and their target configurations, without evaluating specific motion plans between targets. This reduces both the search depth at which plans will be found, and the number of samples required to ensure a plan exists, while crucially preserving correctness guarantees. The result is reduced computational cost of synthesizing plans, and increased robustness of generated plans to actuator noise, model misspecification, or unknown obstacles. Simulation studies show that our hierarchical planning and execution architecture can solve complex navigation and rearrangement tasks, even when faced with narrow passageways or incomplete world information.

==> 1-introduction.tex <==
\section{Introduction}

It has been well-understood for many years that a deliberative planner can make explicit use of a reactive execution layer, for example, a motion primitive library \cite{Majumdar_Tedrake_2017}, in order to simplify the computational burden of planning. However, there has been no way to ensure the correctness of the resulting plan unless the entire trajectory of the motion primitive is evaluated within the planning process, significantly impacting the overall computational cost. This paper shows how a deliberative layer and reactive layer can create abstract plans that are correct-by-construction through the use of continuous constraint contracts (C3) between the layers~\cite{vega-brown2020task}. 

The contract language results in an overall system architecture, shown in Fig. \ref{fig:architecture}, that has several desirable properties. It achieves the computational efficiency that has been seen in many previous task and motion planning approaches,\hl{while being probabilistically complete}. Furthermore, the reactive layer, adapted from our prior work~\cite{vasilopoulos_pavlakos_bowman_caporale_daniilidis_pappas_koditschek_2020}, is robust to environmental uncertainty, and is able to guarantee target convergence and obstacle avoidance, even in the presence of unanticipated obstacles. Importantly, the correctness guarantees of our reactive layer are expressed in terms of well-defined basins of attraction around target configurations, allowing the deliberative layer to simply reason about sequencing isolated targets in the configuration space, without constructing explicit trajectories between them.

% This paper explores how a deliberative planner can make explicit use of a reactive execution layer to simplify its computational burden, extend the scope of and lend robustness to its formal guarantees, in the context of mobile manipulation as depicted in Fig. \ref{fig:minitaur}. 
% Specifically, we construe the basin constructions of the reactive, vector field framework of~\cite{vasilopoulos_pavlakos_bowman_caporale_daniilidis_pappas_koditschek_2020} as instantiating the continuous constraint contracts (C3) representation of~\cite{vega-brown2020task}, and use that subgoal description as the input to a sampling-based domain-independent deliberative planner. 
% The overall system architecture, outlined in Fig.~\ref{fig:architecture}, has several favorable properties.
% First, the {\it deliberative layer} is probabilistically complete and asymptotically optimal, in the sense that as its computational budget increases, it will eventually return the lowest-cost plan that can be expressed as a sequence of behaviors. 
% Second, the {\it reactive layer} guarantees target convergence and avoidance of unforeseen obstacles under specific assumptions about the environment, notably without requiring the deliberative layer to calculate a trajectory to the target, and exposes the capabilities of the underlying robot in terms of well-defined behaviors like grasping, running, and jumping.
% Each of these behaviors can be studied in isolation and included in a low-level {\it gait layer} \cite{topping2019composition}, and several have theoretical proofs of stability and convergence to the desired commands from the reactive layer. 
% Finally, the narrow C3 interface provides explicit means of increasing the scope of the reactive layer to decrease the computational burden of the deliberative layer with respect to task-environment instances that meet the assumptions of the reactive layer's guarantees.
% --- or dialling back up the burden of the computational layer in settings where the reactive layer does not cope as well.

\begin{figure}
  \centering
    \begin{subfigure}[t]{.49\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/minitaur_real.png}
      \caption{The Minitaur platform.}
      \label{fig:minitaur_real}
    \end{subfigure}
    \begin{subfigure}[t]{.47\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/minitaur_gazebo.png}
      \caption{Simulated Minitaur.}
      \label{fig:minitaur_gazebo}
    \end{subfigure}
    \begin{subfigure}[t]{.47\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/toy_example.png}
      \caption{Simple planning problem.}
      \label{fig:toy_problem}
    \end{subfigure}
    \quad
    \begin{subfigure}[t]{.47\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/toy_example_solution.png}
      \caption{Possible goal state.}
      \label{fig:toy_problem_solution}
    \end{subfigure}
  \caption{%
    Top: (a) The physical and (b) simulated Minitaur quadrupedal platform \cite{ghostminitaur}.
    Bottom: (c) An example of a complex dynamically-constrained domain in which a robot must reach the goal region on the lower right, where the heights of the ground plane ($z=0$), the obstacle ($z=1$), and the goal ($z=2$) are all different. The robot can jump only one unit, so the robot must move the cart (red square) to enable a sequence of jumps to reach a goal state (d).
    \label{fig:minitaur}
  }
\end{figure}

\subsection{Motivation and Related Work}

We consider a setting in which a highly energetic quadrupedal robot, capable of behaviors like walking, trotting, jumping and bounding, is assigned various mobile manipulation tasks in an environment cluttered with fixed obstacles and moveable objects (see Fig. \ref{fig:minitaur}). Solving these tasks requires planning and execution of dynamical pedipulation (nonprehensile manipulation of the environment using the robot's general purpose legs)~\cite{Mason_Lynch_1993} as well as more conventional navigation amidst clutter. Developing computationally and physically viable solutions is quite challenging, even assuming a deterministic robot in a fully observable world. Planning entails consideration of each pose of each movable object, the ways in which the robot might affect those poses and the interaction of moving robot-object paths with the fixed obstacles. The order in which objects are moved will generally affect the feasibility of a plan, requiring a combinatorial search. Because the robot dynamics are fast and potentially unstable, integrated feedback and iterated replanning is a virtual necessity if we want to ensure stability and robustness in the face of imperfect geometric (e.g., unanticipated obstacles) and dynamical (e.g., sensor and actuator noise) models.

A large and growing body of work has highlighted the importance of planning representation and good heuristics to address the fundamental complexity of task and motion planning (TAMP) problems like this one. Solutions typically involve a marriage of fast discrete planning tools~\cite{dantam2018incremental} and sampling- or grid-based discretizations of the continuous action space~\cite{garrett2018sampling}, with significant engineering effort going into the design of effective heuristics and sampling strategies that take advantage of both task-level and geometric information~\cite{garrett2020pddlstream,lagriffoul2016combining}. However, while most practical implementations use feedback control to deal with unstable dynamics and sensor uncertainty, there has been little consideration of the ways in which a deliberative planner might rely upon reactive execution to achieve anything more than faithful tracking of the trajectory commands it issues. There are exceptions; preimage back-chaining in deterministic~\cite{LozanoPerez_Mason_Taylor_1984} and stochastic~\cite{kaelbling2017pre} settings aims to guarantee that each prior step of a plan sequence will terminate in a guard condition guaranteeing in turn that the next step of the plan must succeed. Still, notwithstanding a few past examples~\cite{Burridge_Rizzi_Koditschek_1996, Conner_Choset_Rizzi_2009, tedrake2010lqr}, in most systems the computational cost of explicitly determining the basins of attraction (sets of initial conditions from which all trajectories converge to their goals) has cast dubious light on the value of reactive instantiation of a planner's preimages. In addition, these past examples each assume perfect prior information about location and geometry of the workspace and any obstacles.

In our prior work~\cite{Vasilopoulos_Topping_Vega-Brown_Roy_Koditschek_2018}, a deliberative layer produces a sequence of actions and paths, or a \emph{plan}, that if executed perfectly would solve a particular goal specification.
The presence of a vector field based reactive controller then allows a robot to robustly execute these reference actions even in the presence of unanticipated obstacles.
As new obstacles are detected, the world model and reactive controller are updated without requiring the deliberative layer to replan with the new world model.
However, this approach still requires the deliberative planner to sample and validate fine-grained motion primitives to search for a feasible plan to meet the specification, which can be computationally expensive for complex environments where sampling valid action parameters is challenging.

\subsection{Outline of Contributions}

In this work, we leverage the existing assumptions and guarantees for the reactive layer to simplify planning in the deliberative layer, by (i) reducing the overall planning time, (ii) reducing the overall number of planning steps that solve a given problem, and (iii) avoiding continual replanning in the presence of \`a-priori unknown environments. 
By establishing a well-defined {\it contract} between the deliberative and the reactive layer, relying on the fact that the reactive layer can guarantee convergence from any point to any other point within a given connected component of the freespace, we are able to accelerate offline planning and exploit the different (component-wise) formal guarantees of our multi-layer architecture. In particular, the deliberative layer provides guarantees of probabilistic completeness, assuming a perfectly known environment, while the reactive layer ensures collision avoidance and convergence to the target provided by the deliberative layer, even in the presence of unforeseen obstacles.

Focusing on the example of a quadruped robot navigating in an environment with static and movable obstacles, we demonstrate that there are significant computational advantages in the deliberative layer that arise from delegating metric details to the reactive controller.
First, fewer samples are needed for the planner to find a good plan; the difference is especially pronounced when the path requires traversing narrow passages, which are notoriously difficult for sampling-based planners. 
Second, because the deliberative planner is aware of the domain of convergence for each controller and can work out plans using the adjacency relations of the contract basins, it can construct plans with fewer steps than if it relied solely on fine-grained motion primitives --- for example, line-of-sight connections --- and without sacrificing any correctness guarantees. 
The reduction in the length of plans reduces the search depth and dramatically reduces the time required to search for a high-level plan. 
% TODO (nickroy): I think there's an idea missing here, that relates to the highlighted sentence in the lefthand colymn. The deliberative planner could also take advantage of longer motion primitives that don't provide a domain of convergence, but we would give up on guarantees.
Specifically, we show that unburdening the deliberative layer from replanning in the presence of unanticipated obstacles yields dramatic reductions in computational cost (Fig.~\ref{fig:obstacles}), while removing the need to plan motions in connected components of the configuration space yields a computational cost whose exponential growth saturates once the number of movable objects exceeds the number of narrow passages they can obstruct (Fig.~\ref{fig:doorways}). 

More generally, our simulation studies demonstrate that using a hierarchical planning architecture, where the deliberative layer simply reasons about sequencing the contract basins provided by the reactive layer, leads to improvements in computational efficiency for solving complex rearrangement problems entailing dynamic mobile manipulation subgoals, as well as robustness in the face of unforeseen obstacles (Fig.~\ref{fig:dynamic_obstacles}) and imperfect sensorimotor models---all without recourse to fast classical planning algorithms.


\subsection{Organization of the Paper}

The paper is organized as follows. Section~\ref{sec:architecture} describes the proposed multi-layer architecture, along with its component-wise formal guarantees. Section~\ref{sec:domain_description} describes the mobile manipulation problems addressed in this paper, and the specific set of introduced symbolic actions for the Ghost Minitaur robot~\cite{ghostminitaur} used in this study, in two different planning domains for the deliberative planner: a Baseline domain without the reactive planner, employing only simple straight-line motion primitives and used for comparison purposes, and a Reactive domain, employing the proposed architecture. Section~\ref{sec:numerical_experiments} continues with several numerical studies contrasting the performance of the baseline planner with the multi-layer planner, in different scenarios involving simple navigation in \`a-priori known or unknown environments, or mobile manipulation of movable objects in 2D and 2.5D environments. Section~\ref{sec:physical_experiments} provides implementation examples with Minitaur, either in Gazebo or on physical hardware, and, finally, Section~\ref{sec:conclusions} concludes with a summary of the presented work and ideas for future research.

% Specifically, we utilize the assumption that the robot has knowledge of the polygonal objects comprising the world, such that it is always aware of the shape of the current component it inhabits (to enable navigation action in the presence of unknown obstacles) and the components directly adjacent to the current component (to enable manipulation or jumping).
% Then, we utilize the contract (or set of guarantees) provided by the reactive controller: By assuming that the robot can navigate from its current polygonal component to any adjacent polygonal component, we can design a planning domain such that the deliberative layer does not need to sample fine-grained motion primitives, but rather reasons over coarser actions where the robot can move from its current pose to any pose in the current polygon or adjacent polygon through an arbitrarily complex path that the reactive layer is guaranteed to produce (if such a path exists).
% This therefore reduces the depth of plans produced by the deliberative layer and the number of samples needed to find a valid plan, at the expense of performing additional polygon computations per sample to verify the contract between the deliberative and reactive layers.
% As we will later show, these simplifications to the planning domain become particularly effective as the complexity of both anticipated and unanticipated obstacles increases.


==> 3-architecture-v2.tex <==
\section{System Components}
\label{sec:architecture}

This Section describes our modular, multi-layer architecture for planning through contact (Fig.~\ref{fig:minitaur}). 
The architecture consists of deliberative (Section~\ref{sec:deliberative_layer}) and reactive (Section~\ref{sec:reactive_layer}) modules, \hl{which are related via \mbox{{\it contracts}}. The reactive module in turn drives a platform-specific gait layer (Fig.~\mbox{\ref{fig:architecture}}) managing the robot's sensorimotor controls.}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.98\columnwidth]{figures/contract.png}
% \caption{The deliberative and reactive layers communicate by means of a \emph{contract}: the reactive planner guarantees that as long as the initial state satisfies certain \emph{requirements}, then the robot will eventually reach a state satisfying certain \emph{effect} conditions. For example, the reactive layer exposes a {\it ``Walk''} behavior that is guaranteed to reach any specified goal location (red g on the left) from any location for which there is a collision-free path (shaded polygon on the left). This polygon is explicitly computed in the planning loop, and its extent is affected by the state of the world, such as the poses of movable objects (green squares). To implement this behavior, the reactive planner synthesizes a vector field whose basin of attraction spans the set of states for which the requirements are satisfied (right).}
% \label{fig:contract}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%
% DELIBERATIVE LAYER %
%%%%%%%%%%%%%%%%%%%%%%
\subsection{Deliberative layer}
\label{sec:deliberative_layer}
The top layer of our system is a deliberative task and motion planner. 
It is the only element of our planning system that reasons about the entire configuration space, as well as when to make or break contact with objects.

\subsubsection{Inputs and Outputs}
% This layer takes in a description of the world and the capabilities of the reactive layer, as well as a task definition given as a list of constraints on any permissible goal state. It then synthesizes an approximately optimal plan comprising a sequence of actions that can be executed by the reactive layer.  
This layer accepts a description of the world as a collection of objects with geometric information, such as shape and pose, and other properties that constrain the types of actions available with these objects. 
An agent in this world is equipped with parametric actions that can be executed under specific preconditions, and whose outcomes change the state of objects in the world.
Given a task definition, which defines the space of permissible goal states, this layer can synthesize a plan comprising a sequence of actions valid under this world description.

\subsubsection{Description}
\label{sec:deliberative_layer_description}
We use the \emph{continuous constraint contract} (C3) representation for task and motion planning, presented in our prior work~\cite{vega-brown2020task}, to both define the world and capabilities of the reactive layer. 

\textbf{States:} The C3 representation is a continuous extension of the SAS+ formalism \cite{backstrom1995complexity}; as in most planning formalisms, the state of the world is parameterized by the \emph{value} of different \emph{variables}.  A state $\CDRState \in \CDRStates$ is a collection of variable--value pairs, and represents the set of configurations satisfying the constraint defined by the value assigned to each variable. Each variable $v$ corresponds to a function $\eta_v(\mathbf{c})$ mapping configurations $\mathbf{c}$ to an element of the variable's domain; a state $\{v_1 = x_1, v_2 = x_2\}$ describes the set of configurations $\mathbf{c}$ such that $\eta_{v_1}(\mathbf{c}) = x_1$ and $\eta_{v_2}(\mathbf{c}) = x_2$. 
There is no requirement that every variable have an assigned value; variables without values represent inactive constraints. \hl{This implies that a single configuration $\mathbf{c}$ could correspond to multiple states at once; e.g., a configuration $\mathbf{c}$ that satisfies $\eta_{v_1}(\mathbf{c}) = x_1$ and $\eta_{v_2}(\mathbf{c}) = x_2$ corresponds to both states $\{v_1 = x_1, v_2 = x_2\}$ and $\{v_1 = x_1\}$. However, the latter state describes a richer set of configurations, since the constraint related to variable $v_2$ is inactive.}

\hl{In the example shown in Fig.~\mbox{\ref{fig:toy_problem}}, where the problem domain contains a robot and a movable object, the state $\{\texttt{pose}(R)=\robotposition\}$ describes the set of all configurations in which the robot $R$ is at location $\robotposition$, regardless of the pose of the other object \texttt{cart}; the corresponding constraint $\eta_{\texttt{pose}(R)}$ is a projection that extracts the robot's pose from the configuration space. The state $\{\texttt{grasping}(R, \texttt{cart})=1, \texttt{pose}(\texttt{cart})=\robotposition\}$ describes the set of all configurations in which the object is at location $\robotposition$ and the robot is grasping it; the constraint $\eta_{\texttt{grasping}(R,\texttt{cart})}$ could be the distance of the robot from the nearest grasping pose. 

We define the functions $\eta_v$ in terms of domain-specific algorithms for sampling configurations satisfying constraints, though explicit definitions as polynomials or semi-analytic functions are also possible~\mbox{\cite{ vega-brown2020task}}. Following our example, the functions $\eta_{\texttt{pose}(R)}$ and $\eta_{\texttt{grasping}(R, \texttt{cart})}$ are defined implicitly by samplers implemented using computational geometric primitives like collision checking.}

%Both the implicit definition and the continuous variable domains distinguish the C3 representation from most classical planning formalisms.  Defining variables in terms of constraints allows us to reason about continuous domains using a finite symbolic language, without committing \emph{a priori} to a fixed discrete representation. For example, if the problem domain contains a robot and a movable object, the state $\{\texttt{pose}(r)=\robotposition\}$ describes the set of all configurations in which the robot is at location $\robotposition$, regardless of the pose of the other objects; the corresponding constraint $\eta_{\texttt{pose}(r)}$ is a projection that extracts the robot's pose from the configuration space. The state $\texttt{grasping}(r, o)=1, \texttt{pose}(o)=\robotposition$ describes the set of all configurations in which the object is at location $\robotposition$ and the robot is grasping the object; the constraint $\eta_{\texttt{grasping}(r,o)}$ could be the distance of the robot from the nearest grasping pose. 

%In this work, we define the functions $\eta_v$ in terms of domain-specific algorithms for sampling configurations satisfying constraints, though explicit definitions as polynomials or semi-analytic functions are also possible~\cite{ vega-brown2020task}. For example, the functions $\eta_{\texttt{pose}(r)}$ and $\eta_{\texttt{grasping}(r, o)}$ are defined implicitly by samplers implemented using computational geometric primitives like collision checking.

\textbf{Actions:} We define \emph{actions} in this formalism using the behavior classes provided by the reactive layer, where each behavior class $\CDRBareAction$ has a continuous parameterization $\CDRParamSpace_{\CDRBareAction}$. 
For example, \hl{an element $\CDRParams \in \CDRParamSpace_{\CDRBareAction}$ for the navigation action would be a tuple $\{\goalposition, o\}$, with $\goalposition$ and $o$ denoting the target pose to achieve and the object or surface to remain atop respectively.}

Each action represents a contract between the deliberative and reactive layers: formally, we define the requirements and effects of an action $\CDRBareAction$ in terms of two functions \hl{$g_{\CDRBareAction}: \CDRStates \times \CDRParamSpace_{\CDRBareAction} \to \Booleans$} and $f_{\CDRBareAction}: \CDRStates \times \CDRParamSpace_{\CDRBareAction} \to \CDRStates $, where $\CDRStates$ is the space of possible states $\CDRState$. 
The function $g_{\CDRBareAction}(\CDRState, \CDRParams)$ defines the \emph{requirements} of the action, and $f_{\CDRBareAction}(\CDRState, \CDRParams)$ defines its \emph{effects}.
If the system is in state $\CDRState$ when executing action $\CDRBareAction$ with parameters $\CDRParams$, then the reactive planner guarantees that if \hl{$g_{\CDRBareAction}(\CDRState, \CDRParams) = 1$} then at some point in the future the system will reach state $\CDRState' = f_{\CDRBareAction}(\CDRState, \CDRParams)$. 
%In practice, we define $g_{\CDRBareAction}$ and $f_{\CDRBareAction}$ using nonlinear constraints on variable values before and after the action is executed. 
% The search problem can therefore be interpreted as a nonlinear constraint satisfaction problem, where the constraints defined by each action form a constraint graph.
\hl{In our example from Fig.~\mbox{\ref{fig:toy_problem}}, we can define an action $\texttt{jump}(\texttt{from}, \texttt{to}, \robotposition^*)$, parameterized by objects \texttt{from} and \texttt{to} and location $\robotposition^*$, with requirements:}
\begin{enumerate}
    \item \hl{the robot $R$ is at a location $\robotposition$ on top of object \texttt{from}, i.e., $\texttt{atop}(\texttt{pose}(R),\texttt{from})=1$,}
    \item \hl{the location $\robotposition^*$ is on top of object \texttt{to}, i.e., $\texttt{atop}(\robotposition^*,\texttt{to})=1$, and}
    \item \hl{the distance between $\robotposition$ and $\robotposition^*$ is less than a threshold $\epsilon$, i.e., $||\robotposition-\robotposition^*|| \leq \epsilon$.}
\end{enumerate}
\hl{If these requirements are satisfied, the action \texttt{jump} will result in a transition from state $\CDRState := \{\texttt{pose}(R)=\robotposition, \texttt{atop}(\texttt{pose}(R),\texttt{from}) = 1\}$ to new state $\CDRState' := \{\texttt{pose}(R)=\robotposition^*, \texttt{atop}(\texttt{pose}(R),\texttt{to}) = 1\}$.}

By defining actions in terms of constraints, we reduce the problem of planning to finding a sequence of action parameter values that satisfy $g_{\CDRBareAction}$ and intermediate states that constitute effects from $f_{\CDRBareAction}$, a sequence that takes the system from the initial state to a goal state. \hl{However, since states are defined implicitly in terms of variables and their values, a formal definition of the function $f_{\CDRBareAction}$ can be quite hard in practice. Instead, we} solve planning problems defined on a C3 instance using the \hl{sampling-based algorithm} presented in our prior work~\cite{vega-brown2016asymptotically}. We first construct a discrete approximation of the action space by sampling values for the parameters of each action. In navigation or manipulation problems, this generally involves sampling candidate placements for objects or for the robot; importantly, we can sample from the free space of each object independently, rather than sampling from the joint configuration space, without sacrificing completeness or optimality. The sampling process implicitly defines a planning graph: by construction, the finite set of sampled parameters yields a finite (though exponentially large) set of potentially reachable states. Each distinct state is a node in the graph, and there is an edge for each discrete action and state such that the state satisfies the requirements of the action. We then perform a direct heuristic search over this graph to synthesize a plan. We reduce computational cost by considering only a reduced set of constraints in the action requirements when sampling, and checking the remaining constraints only when we find a candidate plan to a given state. Although the graph grows exponentially with number of samples, we typically need to construct and search only a small fraction of the graph.

\subsubsection{Formal guarantees}

\hl{This sampling-based planning algorithm is shown in \mbox{\cite[Theorem 1]{vega-brown2016asymptotically}} to be asymptotically optimal and probabilistically complete, assuming perfect prior knowledge about the environment. In other words, it will either find the shortest-path solution to a TAMP problem or correctly report failure, in the limit of infinite samples. However, in the presence of partially known environments, such as those considered in this work, the notion of ``shortest path'' is not well-defined; the deliberative layer will find a nearly optimal solution given its current estimate about the state of the world, but the reactive layer might choose a longer path during online execution, in order to avoid previously unexpected obstacles. It should be highlighted, however, that probabilistic completeness guarantees are maintained, afforded by our ability to explicitly describe the basin of attraction for each action implemented by the reactive layer, as we will now describe.}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.875\textwidth]{figures/layer_levels.png}
% \caption{
% \textbf{Levels of abstraction in our system architecture.} 
% The deliberative layer reasons about high-level actions like jumping to a pose in an adjacent location, taking into accounts the effects and requirements of that action.
% The reactive layer performs obstacle-aware navigation based on vector fields and a simplified kinematic motion model. 
% The gait layer translates velocity commands from the reactive layer to motion behaviors and detects transitions between regions or with movable objects (using fiducial markers) to trigger transitional behaviors.
% }
% \label{fig:layers}
% \vspace{-13pt}
% \end{figure*}


%%%%%%%%%%%%%%%%%%
% REACTIVE LAYER %
%%%%%%%%%%%%%%%%%%
\subsection{Reactive layer}
\label{sec:reactive_layer}
The reactive layer is responsible for implementing the high-level commands provided by the deliberative layer, and more specifically for handling the geometric details of navigation and manipulation. Rather than instantiating a single motion plan---which could fail in the presence of unanticipated obstacles or unmodeled dynamics---the reactive layer constructs a control policy whose output can be executed by the gait layer and whose execution is guaranteed to achieve the objectives specified by the deliberative layer, or to return with a failure condition expressing the incorrectness of a presumed constraint in the actual environment. 

\subsubsection{Inputs and Outputs}

\hl{Assuming a planar robot, the reactive layer takes as input an estimate of the current reachable set of robot poses, in the form of a polygonal connected component of the robot's workspace, along with a high-level action $\CDRBareAction$ with all parameters $\CDRParams \in \CDRParamSpace_{\CDRBareAction}$ chosen by the deliberative layer. Following our example from Fig.~\mbox{\ref{fig:toy_problem}}, one action in a plan for a rearrangement task, might be $\texttt{push}(\texttt{cart}, \texttt{ground}, \robotposition^*)$ (interpreted as ``push object \texttt{cart} to a target location $\robotposition^*$ atop the object \texttt{ground}'')}. The reactive layer outputs the parameters of a behavior implemented by the gait layer, such as a target velocity and yaw rate. The output parameters vary continuously with the state of the world. 

\subsubsection{Description}

% TODO (wrvb): it's unclear whether from this text whether the reactive layer is limited to navigation or also covers mount/dismount/jump.
The reactive layer is implemented using the vector-field-based feedback motion planning scheme introduced in our prior work~\cite{vasilopoulos_pavlakos_bowman_caporale_daniilidis_pappas_koditschek_2020}. This motion planning scheme is doubly-reactive \cite{Arslan_Koditschek_2018} in the sense that both the trajectory and the vector field are generated online. The critical advantage is that the reactive layer uses a diffeomorphism construction to deform non-convex environments to easily navigable convex worlds, by employing the ``crude'' geometric description of the environment (outer walls) from the deliberative layer together with learned or intrinsic domain specific knowledge about the environment. It is this capacity to plan in a topological model of the encountered geometric environment that enables the reactive layer to describe non-trivial motion through the environment to the deliberative layer in the form of requirements $g_a$ and effects $f_a$.

\textbf{States:} \hl{Unlike the deliberative layer's more general world representation, in the reactive layer we assume that the robot is the only active agent in the world, and} behaves like a first-order, nonholonomically-constrained, disk-shaped robot, centered at location $\robotposition \in \mathbb{R}^2$, with radius $\robotradius \in \mathbb{R}_{>0}$, orientation $\robotorientation \in S^1$ and input vector $\controlunicycle:=(\linearinput,\angularinput)$, consisting of a fore-aft and an angular velocity command. We denote by $\workspace$ the robot's non-convex polygonal workspace, and by $\workspace_{\robotposition} \subseteq \workspace$ the polygonal region corresponding to the space reachable from the robot's current position $\robotposition$. The workspace is cluttered by a finite collection of disjoint obstacles of unknown shape, number, and placement. Similarly, the \textit{freespace} $\freespace$ is defined as the set of collision-free placements for the robot in $\workspace$, and we denote by $\freespace_{\robotposition} \subseteq \freespace$ the freespace component corresponding to $\workspace_{\robotposition}$.

\textbf{Actions:} The reactive controller synthesizes an action as a control law by constructing a diffeomorphism $\diffeogeneric$ between $\freespace_{\robotposition}$ and a convex \emph{model environment}, where non-convex obstacles are either deformed to topologically equivalent disks or merged to the boundary of $\freespace_{\robotposition}$. Then, the robot can navigate by generating virtual commands $\controlunicyclemodel := (\linearinputmodel,\angularinputmodel)$ as in \cite{Arslan_Koditschek_2018}, for an equivalent unicycle model (defined in \cite[Eqs. (24)-(25)]{vasilopoulos_koditschek_2018}) that navigates toward the assigned target position $\goalposition$ in this model environment, and then mapping the virtual commands to physical inputs $(\linearinput,\angularinput)$ through the push-forward of the inverse of $\diffeogeneric$, i.e., $\controlunicycle = \left[ D_{\robotposition} \diffeogeneric \right]^{-1} \controlunicyclemodel$. 

Using the language of the deliberative layer, the requirements $g_a(\robotposition,\goalposition)$ of the navigation action are satisfied if both the robot and target positions are contained in the same component $\freespace_{\robotposition}$ of the robot's freespace. Because we represent the workspace and obstacles using polygons, this calculation can be made using standard tools from computational geometry. More formally, we can decompose $\freespace$ into a finite collection of connected polygons (possibly with holes), and define a set-valued function $\beta_{\freespace}: \freespace \to 2^\freespace$, such that $\freespace_{\robotposition} \triangleq \beta_\freespace(\robotposition) \subseteq \freespace$ is the connected component containing $\robotposition$. \hl{We describe an implementation of this function in Section~\mbox{\ref{sec:global_reactive_planning}}.}

\subsubsection{Formal guarantees}
\label{sec:reactive_layer_guarantees}

\hl{Based on the above description, the online reactive planner guarantees \mbox{\cite[Theorem 2]{vasilopoulos_pavlakos_bowman_caporale_daniilidis_pappas_koditschek_2020}} that if we define $g_a(\robotposition,\goalposition)$ so that it is equal to 1 when $d(\beta_{\freespace}(\robotposition), \beta_{\freespace}(\goalposition)) = 0$ and 0 otherwise (with $d(\cdot, \cdot)$ the distance between sets), then $f_a(\robotposition) \triangleq \goalposition$. In other words, during online execution, the robot will eventually reach $\goalposition$ while avoiding all (previously known or unforeseen) obstacles in the environment, assuming that both the initial robot position $\robotposition$ and the target location $\goalposition$ lie in the same polygonal component $\freespace_{\robotposition}$ of the robot's freespace. This result also holds for rearrangement actions, using the framework in \mbox{\cite{Vasilopoulos_Topping_Vega-Brown_Roy_Koditschek_2018}} for generating virtual commands for the center $\robotposition_{i,c}$ of the circumscribed disk with radius $(\movableobjectradius{i} + \robotradius)$, enclosing the robot and the grasped disk-shaped object with radius $\movableobjectradius{i}$.}

%%%%%%%%%%%%%%
% GAIT LAYER %
%%%%%%%%%%%%%%
% \subsection{Gait layer}
% \label{ref:gait_layer}
% The lowest level of our system, the platform-specific gait layer, uses high-rate feedback control to implement parameterized behavior classes such as walking or jumping. 
% This layer anchors template commands~\cite{Full_Koditschek_1999} received from the reactive layer above it; those commands correspond to behavior classes and include parameters like the target walking speed or yaw rate, and are realized on the robot's joints using low-level sensorimotor feedback from the limb encoders and the onboard IMU. 
% Section \ref{sec:physical_experiments} contains more details on the particular gait layer we use in our experiments.




==> 3-architecture.tex <==
\section{Planning Architecture}
\label{sec:architecture}

In this Section, we describe our modular, multi-layer architecture for planning through contact (see Fig.~\ref{fig:minitaur}). 
The architecture consists of deliberative (Section~\ref{sec:deliberative_layer}) and reactive (Section~\ref{sec:reactive_layer}) modules that communicate via { \em contracts} to drive a platform-specific gait layer (Section~\ref{ref:gait_layer}) that manages the robot's sensorimotor controls.
The actions in the deliberative planner are implemented by the reactive layer as behavior classes designed %
% wrvb: the language here needs finesse; I'd like to say "guaranteed", but we can't.
to converge under well-defined and computationally verifiable conditions on the state of the workspace. 
The contract interface allows us to reason explicitly about these conditions during the planning process, without considering the underlying continuous motion plan. 
It affords the flexibility of passing deliberative plans through to the gait layer when the robot must make or break contracts with objects (e.g., the ``baseline'' mode of interaction detailed in Section~\ref{sec:baseline_domain}) while releasing the deliberative layer from the burden of motion planning when the reactive layer offers a well-characterized basin of attraction around the navigational goal state (e.g., the ``reactive'' mode of interaction detailed in Section~\ref{sec:reactive_domain}).

% TODO (wrvb): While our architecture could be applied to a variety of systems, we focus here on ... 

\begin{figure}[ht]
\centering
\includegraphics[width=1.0\columnwidth]{figures/architecture.png}
\caption{\textbf{System architecture for task and motion planning}. 
A \emph{deliberative layer} searches for a sequence of abstract actions, or a \emph{plan}, that will address a provided task. 
The actions in the plan are passed to a \emph{reactive layer} for robust navigation in complex environments.
This in turn transmits template commands (such as target velocity or a grasp indicator) to a \emph{gait layer} that executes high-rate feedback to achieve parameterized steady-state behaviors on the robot.}
\label{fig:architecture}
\end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.98\columnwidth]{figures/contract.png}
% \caption{The deliberative and reactive layers communicate by means of a \emph{contract}: the reactive planner guarantees that as long as the initial state satisfies certain \emph{requirements}, then the robot will eventually reach a state satisfying certain \emph{effect} conditions. For example, the reactive layer exposes a {\it ``Walk''} behavior that is guaranteed to reach any specified goal location (red g on the left) from any location for which there is a collision-free path (shaded polygon on the left). This polygon is explicitly computed in the planning loop, and its extent is affected by the state of the world, such as the poses of movable objects (green squares). To implement this behavior, the reactive planner synthesizes a vector field whose basin of attraction spans the set of states for which the requirements are satisfied (right).}
% \label{fig:contract}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%
% DELIBERATIVE LAYER %
%%%%%%%%%%%%%%%%%%%%%%
\subsection{Deliberative layer}
\label{sec:deliberative_layer}
The top layer of our system is a deliberative task and motion planner. 
It is the only element of our planning system that reasons about the entire configuration space, as well as when to make or break contact with objects.

\subsubsection{Inputs and Outputs}
% This layer takes in a description of the world and the capabilities of the reactive layer, as well as a task definition given as a list of constraints on any permissible goal state. It then synthesizes an approximately optimal plan comprising a sequence of actions that can be executed by the reactive layer.  
This layer accepts a description of the world as a collection of objects with geometric information, such as shape and pose, as well as other properties that constrain the types of actions available with these objects. 
An agent in this world is equipped with a set of parametric actions that can be executed under specific preconditions, and whose outcomes change the state of objects in the world.
Given a task definition, which is a list of constraints defining the space of permissible goal states, this layer can synthesize an approximately optimal plan comprising a sequence of actions valid under this world description.

\subsubsection{Description}
We use the \emph{continuous constraint contract} (C3) representation for task and motion planning, presented in our prior work~\cite{vega-brown2020task}, to both define the world and capabilities of the reactive layer. The C3 representation is a continuous extension of the SAS+ formalism \cite{backstrom1995complexity}; as in most planning formalisms, the state of the world is parameterized by the \emph{value} of different \emph{variables}. The state representation differs from most classical planning formalisms in two ways: first, the values are drawn from arbitrary continuous domains; and second, variable values are interpreted as \emph{constraints} on the set of possible configurations of the world. For example, to model a world with three objects $\{o_1, o_2, o_3\}$ our planning domains include variables $\texttt{pose}(o)$ for the pose of each object $o$ in some absolute coordinate frame. While pose variables are sufficient for geometric planning, we also enrich our domain representations with other variables like $\texttt{atop}(o, o')$ to denote the set of configurations in which object $o$ is resting on object $o'$. A state is a collection of variable-value pairs, and represents the set of configurations satisfying the constraint defined by the value assigned to each variable. There is no requirement that every variable have an assigned value; variables without values represent inactive constraints.
% wrvb: added details about how the representation can be richer than just *poses*, and how constraints combine to form states.

We define \emph{actions} in this formalism using the behavior classes provided by the reactive layer, where each behavior class of the reactive layer has a continuous parameterization. 
For example, navigation is modeled by an action parameterized by the target location, and is implemented with a behavior class designed to reach the target location while avoiding obstacles, provided it is possible to do so without manipulating any movable objects.
Each action represents a contract between the deliberative and reactive layers: the reactive planner guarantees that if certain \emph{requirements} hold in terms of the world state variables, then there is an executable policy that will terminate in finite time, incur only bounded cost, and ensure that certain \emph{effect} conditions hold on the world state variables. 

Formally, we define the requirements and effects of an action $\CDRBareAction$ in terms of two functions $f_{\CDRBareAction}: \CDRStates \times \CDRParamSpace_{\CDRBareAction} \to \CDRStates $ and $g_{\CDRBareAction}: \CDRStates \times \CDRParamSpace_{\CDRBareAction} \to \Reals$, where $\CDRParamSpace_{\CDRBareAction}$ is the space of parameters of the action $\CDRBareAction$, and $\CDRStates$ is the space of possible states. 
The function $f_{\CDRBareAction}(\CDRState, \CDRParams)$ defines the \emph{effects} of the action, and $g_{\CDRBareAction}(\CDRState, \CDRParams)$ defines the \emph{requirements} of the action.
If the system is in state $\CDRState$ when the reactive planner executes action $\CDRBareAction$ with parameters $\CDRParams$, then the reactive planner guarantees that if $g_{\CDRBareAction}(\CDRState, \CDRParams) \ge 0$ then at some point in the future the system will reach state $\CDRState' = f_{\CDRBareAction}(\CDRState, \CDRParams)$. 
In practice, we define $f_{\CDRBareAction}$ and $g_{\CDRBareAction}$ using nonlinear constraints on variable values before and after the action is executed. 
By defining actions in terms of constraints, we reduce the problem of planning to finding a sequence of action parameter values and intermediate states which take the system from the initial configuration to an acceptable goal state. The search problem can therefore be interpreted as a nonlinear constraint satisfaction problem, where the constraints defined by each action form a constraint graph. With care, action contracts can be designed to keep this constraint graph sparse, minimizing the number of variables involved in each action. 

We solve planning problems defined on a C3 instance using the asymptotically-optimal sampling-based planning algorithm presented in our prior work~\cite{vega-brown2016asymptotically}. We first construct a discrete approximation of the action space by sampling possible values for the parameters of each action. The sampling process implicitly defines a planning graph: by construction, the finite set of sampled parameters yields a finite (though exponentially large) set of potentially reachable states. Each distinct state is a vertex in the graph, and there is an edge for each discrete action and state such that the state satisfies the requirements of the action. We then perform a direct heuristic search over this graph to synthesize a plan.

In our previous work, the constraints $f_{\CDRBareAction}$ and $g_{\CDRBareAction}$ were taken to be simple geometric primitives. For example, a navigation action would succeed if the straight-line path to the target pose was collision free.  In this work, we show that we can use properties of the behavior classes of the reactive layer to define a much richer set of constraints. %
% wrvb: again, I want to say "provable properties" but don't think we can.
For example, as described in Section~\ref{sec:reactive_layer}, the goal conditions of the reactive planning behavior do not require a straight-line collision-free path, but merely that the topology of the surrounding environment allows a diffeomorphism to be constructed to a convex world.  We can construct such a diffeomorphism explicitly, and the construction depends only on the location of movable objects and not on the state of the robot---meaning that we need compute the construction only once, and can search for plans without repeatedly invoking a low-level motion planner.

The flexibility to plan with arbitrary constraints, along with the existence of a rich set of contracts defined by computationally-inexpensive constraints, allows the hierarchical architecture to abstract away many of the details of the lower level plan while still ensuring correctness: any plan generated by the deliberative planner is guaranteed to be executable by the reactive layer.
The abstraction of geometric details allows us to reduce not only the number of actions to be considered for each plan, but also the number of sampled parameters for each action---and permits the hierarchical planning system to find complex plans via direct search, even without leveraging fast planning heuristics.
% wrvb: removed "far more readily", which invites the question, than what?
% kod: Please see if you find my distinction between topological vs geometrically-instantiated planning to be appropriate
%   TODO (wrvb): unclear what that means in this context?

To further reduce computational complexity, we construct our discrete approximation lazily by considering only a reduced set of constraints in the behavior contracts when sampling, and checking the remaining constraints only when we find a candidate plan to reach a given state. Consequently, even though the graph grows exponentially with the number of samples, we typically need to construct and search only a small fraction of the graph, while still preserving the optimality guarantees provided by the combination of the reactive layer behavior classes and the contracts the deliberative planner honors when calling those behavior classes.


%%%%%%%%%%%%%%%%%%
% REACTIVE LAYER %
%%%%%%%%%%%%%%%%%%
\subsection{Reactive layer}
\label{sec:reactive_layer}
The reactive layer is responsible for implementing the high-level commands provided by the deliberative layer, and more specifically for dealing with the geometric details of navigation. Rather than instantiating a single motion plan---which could fail in the presence of unanticipated obstacles or unmodeled dynamics---the reactive layer constructs a control policy whose output can be executed by the gait layer and whose execution is guaranteed to achieve the objectives specified by the deliberative layer. 

\subsubsection{Inputs and Outputs}

The reactive layer takes as input an estimate of the current state of the world along with a high-level action description with all parameters instantiated. For example, one action in a plan for a rearrangement task, might be $\texttt{push}(o, x)$ (interpreted as ``push object $o$ to a target location $x$''). The input actions, and their parameterizations, are exactly the same as in the deliberative layer.

The reactive layer outputs the parameters of a behavior implemented by the gait layer, such as a target velocity and yaw rate for navigation. The output parameters vary continuously with the state of the world. The reactive layer acts as a feedback controller, handling both expected and unexpected changes in the world state and guaranteeing convergence to a state satisfying the effect constraints of the high-level action. 
While the space of parameters depends on the low-level behavior being executed, in our implementation the reactive outputs are either \begin{itemize}
  \item a differential drive template command corresponding to the intended behavior class for the physical robot to execute when navigating the workspace with or without a grasped object, or 
  \item an appropriately defined command for a transitional robot maneuver (e.g., the height of the platform that the robot needs to scale, or the distance from the object it needs to manipulate). 
\end{itemize}

\subsubsection{Description}

% TODO (wrvb): it's unclear whether from this text whether the reactive layer is limited to navigation or also covers mount/dismount/jump.
The reactive layer is implemented using the vector field-based feedback motion planning scheme introduced in our prior work~\cite{vasilopoulos_pavlakos_bowman_caporale_daniilidis_pappas_koditschek_2020}. This scheme guarantees target convergence and obstacle avoidance in unexplored environments by employing a combination of an onboard LIDAR and an RGB camera for obstacle identification and localization. This motion planning scheme is doubly-reactive \cite{Arslan_Koditschek_2018} in the sense that both the trajectory and the vector field are generated online, and uses a diffeomorphism construction in order to deform non-convex environments to easily navigable convex worlds, by employing the ``crude'' geometric description of the environment (outer walls) from the deliberative layer. Moreover, the reactive layer localizes movable objects in the workspace (by using assigned AprilTags \cite{wang2016iros}), and accordingly updates the assumed object locations to properly approach and jump on a fixed or movable platform, or grasp a movable object. Finally, except for simple navigation tasks, the reactive layer is responsible for following desired symbolic action targets when gripping and manipulating movable objects (see \cite{Vasilopoulos_Topping_Vega-Brown_Roy_Koditschek_2018}). 

Although the input actions are defined and parameterized exactly as they are in the deliberative layer, the world representation used in the reactive layer differs from the deliberative world model: it incorporates a model of continuous dynamics, it can include obstacles not modeled in the deliberative layer, and it uses a simplified geometric model in which the robot and all movable objects are disk-shaped. The internal world models of the reactive and deliberative layers need only be compatible enough that the reactive layer can guarantee adherence to the contract defining the high-level action. % wrvb: too wordy

Concretely, in the reactive layer we assume that our robot behaves like a first-order, nonholonomically-constrained, disk-shaped robot, centered at $\robotposition \in \mathbb{R}^2$, with radius $\robotradius \in \mathbb{R}_{>0}$, orientation $\robotorientation \in S^1$ and input vector $\controlunicycle:=(\linearinput,\angularinput)$, consisting of a fore-aft and an angular velocity command. The workspace is cluttered by a finite collection of disjoint obstacles of unknown number and placement, denoted by $\obstacleset$. This set might also include non-convex ``intrusions'' of the boundary of the physical workspace $\workspace$ into the convex hull of the closure of the workspace $\workspace$, defined as the {\it enclosing workspace}. Similarly, the \textit{freespace} $\freespace$ is defined as the set of collision-free placements for the robot, and the \textit{enclosing freespace}, $\enclosingfreespace$, is defined as $\enclosingfreespace := \left\{ \robotposition \in \mathbb{R}^2 \, | \, \robotposition \in \text{Conv}(\overline{\freespace}) \right\}$.

The main idea of the reactive controller is to synthesize a control law by constructing a diffeomorphism $\diffeogeneric$ between the physical environment and a convex \emph{model environment}, % wrvb: switched word order to avoid confusing readers who parse "model" as a noun instead of an adjective 
whose boundary is the enclosing freespace, $\enclosingfreespace$, and where non-convex obstacles are either deformed to topologically equivalent disks or merged to $\enclosingfreespace$. Then, the robot can navigate by generating virtual commands $\controlunicyclemodel := (\linearinputmodel,\angularinputmodel)$ in this model environment (which is simple, as the transformed freespace is convex), and map the virtual commands to physical inputs $(\linearinput,\angularinput)$ through the push-forward of the inverse of $\diffeogeneric$, i.e., $\controlunicycle = \left[ D_{\robotposition} \diffeogeneric \right]^{-1} \controlunicyclemodel$.

This idea can be extended to handle rearrangement actions. The robot is assumed to use a gripper to move disk-shaped {\it movable objects} of known location, denoted by $\movableobjectset:=\{\movableobject_i\}_{i \in \{1,\ldots,\movableobjectcardinality\}}$, with a vector of radii $(\movableobjectradius{1}, \ldots, \movableobjectradius{\movableobjectcardinality}) \in \mathbb{R}^{\movableobjectcardinality}$, in a closed, compact, polygonal, typically non-convex workspace $\workspace \subset \mathbb{R}^2$. The physical platform does not possess an actual gripper (see Fig. \ref{fig:minitaur}); the gait layer must coordinate the robot's joints so that the front limbs behave like a virtual gripper.

When the robot is gripping an object $i$, we use the method from \cite{Vasilopoulos_Topping_Vega-Brown_Roy_Koditschek_2018} for generating virtual commands for the center $\robotposition_{i,c}$ of the circumscribed disk with radius $(\movableobjectradius{i} + \robotradius)$, enclosing the robot and the object. Namely, we assume that the robot-object pair is a fully actuated particle with dynamics $\dot{\robotposition}_{i,c} = \controlfullyactuated_{i,c}(\robotposition_{i,c})$, design our control policy $\controlfullyactuated_{i,c}$ using the same vector field controller, and translate to commands $\controlunicycle = (\linearinput,\angularinput)$ for our differential drive robot as $\controlunicycle := \mathbf{T}_{i,c}(\robotorientation)^{-1} \, \controlfullyactuated_{i,c}$, with $\mathbf{T}_{i,c}(\robotorientation)$ the Jacobian of the gripping contact, i.e., $\dot{\robotposition}_{i,c} = \mathbf{T}_{i,c}(\robotorientation) \, \controlunicycle$.

%%%%%%%%%%%%%%
% GAIT LAYER %
%%%%%%%%%%%%%%
\subsection{Gait layer}
\label{ref:gait_layer}
The lowest level of our system, the platform-specific gait layer, uses high-rate feedback control to implement parameterized behavior classes such as walking or jumping. 

\subsubsection{Inputs and Outputs}
This layer anchors template commands~\cite{ Full_Koditschek_1999,Culbertson_Gustafson_Koditschek_Stiller_2020} received from the reactive layer above it; those commands correspond to behavior classes and include parameters like the target speed or yaw rate while walking, and are realized on the robot's joints using low-level sensorimotor feedback from the limb encoders and the onboard IMU.

\subsubsection{Description}
The gait layer abstracts the details of determining how the limbs should move or how to negotiate uneven terrain, freeing the reactive planner to determine how to achieve local goals for placements of the body and movable objects in the world. For our quadruped experiments, we employ the steady-state behaviors {\it ``Walk''} and {\it ``Push-Walk''} from~\cite{Vasilopoulos_Topping_Vega-Brown_Roy_Koditschek_2018}, to either navigate the workspace or use the robot's front limbs as a virtual gripper when manipulating movable objects respectively. 
In addition, we use a set of four transitional behaviors: {\it ``Mount''}, {\it ``Dismount''}, {\it ``Jump-Up''} and {\it ``Jump-Across''}, adapted from~\cite{topping2019composition}, to mount and dismount objects, or jump on top of platforms or across gaps. 
A detailed description of the control scheme used to realize the abstract template commands is beyond the scope of the present paper.

\subsection{Formal Guarantees}

The hierarchical planning framework described in this section largely preserves the formal guarantees of its constituent layers.
Specifically, the deliberative planning framework is both probabilistically complete and asymptotically optimal, and will only return feasible plans; consequently, whenever the reactive layer can guarantee completeness (anything the robot can achieve can be achieved by a sequence of reactive behaviors) and convergence (all behaviors are guaranteed to reach a terminating set in finite time), the hierarchical system is probabilistically complete. 
In addition, whenever the reactive layer can guarantee optimality (any behavior the robot is capable of can be approximated arbitrarily well as a sequence of reactive behaviors), the hierarchical system is asymptotically optimal.
% TODO (wrvb): does this require proof or citation? If so my thesis is probably the cleanest reference.

% As a motivating example, consider a trivial implementation of the action \texttt{move}, parameterized by a target location $t$, which requires that the straight-line path from the robot's initial pose $x$ to $t$ is collision-free, and ensures the robot will be located at $t$ when the action ends. In this example, $f_{\CDRBareAction}(\CDRState, \CDRParams)$ would be defined so that the value of the robot pose is equal to $\CDRParams$, and the value of every other variable is unchanged, and $g_{\CDRBareAction}(\CDRState, \CDRParams)$ would be defined as the smallest distance between the robot geometry and any stationary or movable object as the robot moves from its initial location to $\CDRParams$. Then, as long as the deliberative planner calls the \texttt{move} action only from poses $x$ with parameters $t$ where the straight-line path is collision-free, a high-level plan consisting of such move actions will be (i) complete, (ii) correct, and (iii) asymptotically optimal in the limit of infinite samples.

We observe that the reactive controller guarantees target convergence and collision avoidance for both a single differential drive robot and a differential drive robot gripping and manipulating objects when both the initial position of the robot $\robotposition$ (or the robot-object pair center $\robotposition_{i,c}$ for an object $i$) and the target location $\goalposition$ lie in the same connected component of a 2D workspace. Consequently, if the deliberative layer supplies a freespace connected component $\freespace$ that includes the robot's location, along with a symbolic action that requires the robot to visit, grasp, or release a target object within the same region, the reactive controller can find the enclosing freespace $\enclosingfreespace$, construct the diffeomorphism $\diffeogeneric$, and guarantee the successful execution of the action. It follows that for rearrangement tasks the reactive layer can guarantee convergence and completeness, and thus the hierarchical system is probabilistically complete. This statement holds even in the presence of unknown and unanticipated obstacles, without deliberative replanning, provided any unanticipated obstacles are well-separated in a precise sense described in~\cite{vasilopoulos_pavlakos_bowman_caporale_daniilidis_pappas_koditschek_2020}. 

% TODO: kod asks for f and g functions here---not sure how best to explain them without reference to domain?

% TODO: we might consider alluding to other claims we think are true. 
%   cf kod's "Crucial to articulate this as formally as possible---even perhaps
%   making explicitly conjectural ("to-be-proven-in-the-future") statements"

